AMICO: Amodal Instance Composition

Image composition aims to blend multiple objects to form a harmonized image. Existing approaches often assume precisely segmented and intact objects. Such assumptions, however, are hard to satisfy in unconstrained scenarios. We present Amodal Instance Composition for compositing imperfect -- potentially incomplete and/or coarsely segmented -- objects onto a target image. We first develop object shape prediction and content completion modules to synthesize the amodal contents. We then propose a neural composition model to blend the objects seamlessly. Our primary technical novelty lies in using separate foreground/background representations and blending mask prediction to alleviate segmentation errors. Our results show state-of-the-art performance on public COCOA and KINS benchmarks and attain favorable visual results across diverse scenes. We demonstrate various image composition applications such as object insertion and de-occlusion.

==> figure_latex/04-amo-content.tex <==
d\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figure/am_content.pdf}
\begin{minipage}{\linewidth}
% \centering
\hspace{1cm} Original \hspace{1cm}
De-occ.~\cite{zhan2020self} \hspace{1cm} Ours
\end{minipage}
\caption{
\textbf{Visual comparison of amodal instance segmentation and content prediction.} For each paired rows, we show the original images and the corresponding amodal annotation (left) and the results of predicted amodal masks~\textit{(Row 1,3)} and synthetic de-occluded objects~\textit{(Row 2,4)} by ~\cite{zhan2020self} (middle) and ours (right).
\ck{This also requires some work, but I don't know the method well and am hesitant to edit it myself.}
}
\label{fig:am_content}
\end{figure}



==> figure_latex/comp_generalization.tex <==

\begin{figure}[t]
\centering
\begin{minipage}{\linewidth}
\centering
\includegraphics[width=.9\linewidth]{figure/painting_bg.pdf}
\end{minipage}
\begin{minipage}{\linewidth}
\centering
Cut-n-paste 
\hspace{.23\linewidth} Composed result
% \vspace{-.2cm}
\end{minipage}

\vspace{0.2cm}
\caption{\textbf{Neural compositing results with \emph{painting} background}: We experiment with blending objects to \emph{out-of-domain} (never seen during training) scenarios to test the generalization capability of our method. We show compositions onto paintings with different styles.
% (\textit{left}) cut-and-paste images; (\textit{right}) composed results by our neural compositing model.
}
%\vspace{-0.2cm}
\label{fig:painting}
\end{figure}


==> figure_latex/completion_gt.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figure/content_gt.pdf}
    \begin{minipage}{\linewidth}
    % \centering
    \hspace{0.1cm} Masked image\hspace{0.7cm}
    GConv~\cite{yu2019free} \hspace{0.7cm} CRA~\cite{yi2020contextual}\hspace{1cm}
    IIC~\cite{zeng2020high}\hspace{0.8cm}  
    EdgeCon.~\cite{nazeri2019edgeconnect}\hspace{1cm}
    Ours\hspace{1cm} Ground truth
    \end{minipage}
    \caption{\textbf{Visual comparison of Object completion for masked instances.} 
    Given an image (\textit{col.7}) as well as object masks, our method inpaints the occluded part of the objects (\textit{col.1}, marked in yellow).
    % The completion results by different methods are shown in column 2-5. 
    }
    \vspace{-0.3cm}
    \label{fig:obj_completion_gt}
\end{figure*}

